Profile-Based Privacy for Locally Private Computations

Differential privacy has emerged as a gold standard in privacy-preserving data analysis. A popular variant is local differential privacy, where the data holder is the trusted curator. A major barrier, however, towards a wider adoption of this model is that it offers a poor privacy-utility tradeoff. In this work, we address this problem by introducing a new variant of local privacy called profile-based privacy. The central idea is that the problem setting comes with a graph G of data generating distributions, whose edges encode sensitive pairs of distributions that should be made indistinguishable. This provides higher utility because unlike local differential privacy, we no longer need to make every pair of private values in the domain indistinguishable, and instead only protect the identity of the underlying distribution. We establish privacy properties of the profile-based privacy definition, such as post-processing invariance and graceful composition. Finally, we provide mechanisms that are private in this framework, and show via simulations that they achieve higher utility than the corresponding local differential privacy mechanisms.

==> macro.tex <==
\usepackage{amsmath,amssymb, amsthm}
\usepackage[utf8]{inputenc}

%\usepackage{natbib}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{fullpage}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{color}
\usepackage{mdframed}

\widowpenalty10000
\clubpenalty10000

%\renewcommand{\topfraction}{.85}
%\renewcommand{\bottomfraction}{.7}
%\renewcommand{\textfraction}{.15}
%\renewcommand{\floatpagefraction}{.66}
%\renewcommand{\dbltopfraction}{.66}
%\renewcommand{\dblfloatpagefraction}{.66}
%\setcounter{topnumber}{9}
%\setcounter{bottomnumber}{9}
%\setcounter{totalnumber}{20}
%\setcounter{dbltopnumber}{9}

%\renewcommand{\labelitemi}{\textbullet}
%\renewcommand{\labelitemii}{\textbullet}
%\renewcommand{\labelitemiii}{\textbullet}
%\renewcommand{\labelitemiv}{\textbullet}
\usepackage{enumitem}
\setlistdepth{9}

%\setlist[itemize,1]{label=$\bullet$}
%\setlist[itemize,2]{label=$\bullet$}
%\setlist[itemize,3]{label=$\bullet$}
%\setlist[itemize,4]{label=$\bullet$}
%\setlist[itemize,5]{label=$\bullet$}
%\setlist[itemize,6]{label=$\bullet$}
%\setlist[itemize,7]{label=$\bullet$}
%\setlist[itemize,8]{label=$\bullet$}
%\setlist[itemize,9]{label=$\bullet$}
\setlist[itemize,1]{label=$ $}
\setlist[itemize,2]{label=$ $}
\setlist[itemize,3]{label=$ $}
\setlist[itemize,4]{label=$ $}
\setlist[itemize,5]{label=$ $}
\setlist[itemize,6]{label=$ $}
\setlist[itemize,7]{label=$ $}
\setlist[itemize,8]{label=$ $}
\setlist[itemize,9]{label=$ $}


\renewlist{itemize}{itemize}{9}

\newtheorem{Thm}{Theorem}
\newtheorem{Lem}[Thm]{Lemma}
\newtheorem{Cor}[Thm]{Corollary}
\newtheorem{Prop}[Thm]{Proposition}
\newtheorem{Claim}[Thm]{Claim}
\newtheorem{lemma}{Lemma}
\newtheorem{Observation}{Observation}
\newtheorem{theorem}{Theorem}
\newenvironment{proof2}{\noindent {\sc Proof:}}{$\Box$ \medskip} %renamed due to amsthm package also defining proof, but I like the QED symbol here better.-Jimmy
\newtheorem{Ex}{Exercise}
\newtheorem{Exa}{Example}
\newtheorem{Rem}{Remark}
\newtheorem{assumption}{Assumption}

%\theoremstyle{}
%\newtheorem{Defn}{Definition}
%\newmdtheoremenv{Defn}{Definition}
%\theoremstyle{plain}

\newcommand{\calC}{{\mathcal{C}}}
\newcommand{\calA}{{\mathcal{A}}}
\newcommand{\calP}{{\mathcal{P}}}
\newcommand{\calO}{{\mathcal{O}}}
\newcommand{\kc}[1]{\noindent {\color{red}{{\smallskip \textbf{KC: }}#1}}}
\newcommand{\jg}[1]{\noindent {\color{blue}{{\smallskip \textbf{JG: }}#1}}}

\newcommand{\bbR}{{\mathbf{R}}}
\newcommand{\disth}[1]{d_{\operatorname{ham}}(#1)}
\newcommand{\distp}[1]{d_{\operatorname{prok}}(#1)}
\newcommand{\calX}{{\mathcal{X}}}
\newcommand{\calY}{{\mathcal{Y}}}

\newcommand{\calF}{{\mathcal{F}}}
\newcommand{\bbE}{{\mathbb{E}}}
\def\calN{\mathcal{N}}
\newcommand{\err}{\mathbf{err}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calD}{\mathcal{D}}
%\renewcommand{\Pr}[1]{\underset{#1}{\text{Pr}}}
\renewcommand{\Pr}{\text{Pr}}
\def\Lap{\mathbf{Lap}}
\def\Exp{\mathbf{Exp}}
\def\Beta{\mathbf{Beta}}
\def\dx{\mathrm{d}}
\def\argmax{\mathrm{argmax}}
\def\argmin{\mathrm{argmin}}
\def\tln{\tilde{n}}
\def\E{\mathbb{E}}
\def\Dfam{\mathbb{D}}

\def\T{\mathbf{T}}
\def\x{\mathbf{x}}
\def\X{\mathbf{X}}

\def\Diff{Diff} %Difference set, perhaps change to \Delta_{\calX}

\usepackage{xr}


%theorem numbering for appendices - Jimmy
\usepackage{chngcntr}
\usepackage{apptools}
\AtAppendix{\counterwithin{theorem}{section}}
\usepackage{geometry}

%%%%%%%% above copied from main.tex %%%%%%%%%%%











%\documentclass[11pt]{article}
%\usepackage[margin=1in]{geometry}
% use Times
%\usepackage{times}
%% For figures
%\usepackage{graphicx} % more modern
%%\usepackage{epsfig} % less modern
%\usepackage{subcaption} 
%
%% For citations
%\usepackage{natbib}
%
%% For algorithms
%\usepackage{hyperref}
%\usepackage{url}
%\usepackage{graphicx}
%\usepackage{amsfonts}
%\usepackage{amsmath}
%\usepackage{amsthm}
%
%\usepackage{algorithm}
%\usepackage{algorithmic}
%%\usepackage{algpseudocode}
%
%\newcommand{\fix}{\marginpar{FIX}}
%\newcommand{\new}{\marginpar{NEW}}
%\newcommand*\diff{\mathop{}\!\mathrm{d}}
%\newcommand*\Diff[1]{\mathop{}\!\mathrm{d^#1}}
%\newcommand{\calF}{\mathcal{F}}
%\newcommand{\calD}{\mathcal{D}}
%\newcommand{\calM}{\mathcal{M}}
%\newcommand{\Lap}{\text{Lap}}
%\newcommand{\card}[1]{\texttt{card}(#1)}
%
\usepackage[usenames, dvipsnames]{xcolor}
%\newcommand{\kc}[1]{{\textcolor{red}{#1}}}
\newcommand{\shs}[1]{{\textcolor{NavyBlue}{SS: #1}}}
%\newcommand{\rmk}[1]{{\textcolor{ForestGreen}{RMK: #1}}}
%\newcommand{\notshow}[1]{}
%\def\calS{\mathcal{S}}
%\def\calQ{\mathcal{Q}}
%\def\calX{\mathcal{X}}
%\def\Ni{{N\backslash\{i\}}}
%
%%\newcommand{\calR}{\mathcal{R}}
%%\newcommand{\calN}{\mathcal{N}}
%%\newcommand{\XR}{X_\mathcal{R}}
%%\newcommand{\XN}{X_\mathcal{N}}
%
%\newcommand{\basicAlgo}{\text{BasicMarkovQuiltMechansim}}
%\newcommand{\fastAlgo}{FastMarkovQuiltMechanism}
%\newcommand{\subroutine}{\text{FindBestMarkovQuilt}}
%\def\mqm{\text{Markov Quilt Mechanism}}
%\newcommand{\MQM}{\text{MQM}}
%\def\calY{\mathcal{Y}}
%\def\g{g}
%\def\FA{\mathcal{F}_{\mathcal{A}}}
%\def\FB{\mathcal{F}_{\mathcal{B}}}
%\def\XA{{X}^{\mathcal{A}}}
%\def\XB{{X}^{\mathcal{B}}}
%\def\xA{{x}^{\mathcal{A}}}
%\def\xB{{x}^{\mathcal{B}}}
%\def\ZA{{Z}_{\mathcal{A}}}
%\def\ZB{{Z}_{\mathcal{B}}}
%\def\wA{{w}_{\mathcal{A}}}
%\def\wB{{w}_{\mathcal{B}}}
%\def\SA{{S}_{\mathcal{A}}}
%\def\SB{{S}_{\mathcal{B}}}
%\def\QA{{Q}_{\mathcal{A}}}
%\def\QB{{Q}_{\mathcal{B}}}
%\def\epsilonA{{\epsilon_{\mathcal{A}}}}
%\def\epsilonB{{\epsilon_{\mathcal{B}}}}
%\def\RQ{{R\cup Q}}
%\def\inner{\text{in}}
%\def\out{\text{out}}
%\def\MA{\mathcal{M_A}}
%\def\MB{\mathcal{M_B}}
%
%\newcommand{\Dinf}[2]{D_{\infty}\big(#1 ~\|~ #2\big)}
%
%
%\newtheorem{theorem}{Theorem}[section]
\newtheorem{Defn}[theorem]{Definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{observation}[theorem]{Observation}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{claim}[theorem]{Claim}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{condition}[theorem]{Condition}
%
%\def\effect{max-influence}
%
%\renewcommand{\Pr}[2]{\mathbb{P}_{#1}\left[ #2 \right]}
\renewcommand{\exp}[1]{\text{exp}\left( #1 \right)}
\newcommand{\Expect}[2]{\mathbb{E}_{#1}\left[ #2 \right]}
\newcommand{\KL}[2]{D_{\text{KL}} \left(#1 \| #2\right)}
%\newcommand{\erf}[1]{\text{erf} \left(#1 \right)}
%\newcommand{\GammaF}[1]{\Gamma \left(#1 \right)}
%\newcommand{\GammaFF}[2]{\Gamma \left(#1, #2\right)}
%\newcommand{\F}[3]{F_1 \left(#1; #2; #3 \right)}

\newcommand{\reg}{\beta}
\newcommand{\renyi}[3]{D_{#1}\left(#2 \| #3\right)}
\renewcommand{\ln}[1]{\log\left(#1\right)}
\newcommand{\rdp}{\text{RDP}}
\newcommand{\rd}{\text{R\'enyi Divergence}}
\usepackage{bbm}
\newcommand{\ind}[1]{\mathbbm{1}\left(#1\right)}



==> related.tex <==
\section{Related Work}

Our proposed definition shares ideas behind two commonly used privacy frameworks: the generalized Pufferfish privacy framework~\cite{KM12}, and geoindistinguishability~\cite{geoind13}. Like our definition, Pufferfish presents an explicit separation of sensitive and insensitive information with distributional assumptions. However, we focus on a local case with distributional secrets, while the existing Pufferfish literature targets value-dependent secrets. The flexible privacy specification also makes our defintion similar to geoindistinguishability, but our work does not require an explicit metric and applies more readily to a discrete setting.

Our methods also resemble those seen under maximal-leakage-constrained hypothesis testing~\cite{liao2017hypothesis}. The maximal-leakage framework also employs a distribution-focused mechanism design, but solves a different problem. Our work aims to prevent identifying distributions while preserving and identifying observed values where possible. The maximal-leakage setting inverts this goal, and protects the observed values. This distinction in goal also applies with respect to the distributional privacy framework~\cite{balcan2012distributed}.

Our work can also be viewed in relation to information theoretic definitions dues to the deep connections present from differential privacy. We do not directly comment on these connections in this work, and instead focus on how our definition appears from the lens of differential privacy.\

